Cryptographic Characterization of Quantum Advantage

Quantum computational advantage refers to an existence of computational tasks that are easy for quantum computing but hard for classical one. Unconditionally showing quantum advantage is beyond our current understanding of complexity theory, and therefore some computational assumptions are needed. Which complexity assumption is necessary and sufficient for quantum advantage? In this paper, we show that inefficient-verifier proofs of quantumness (IV-PoQ) exist if and only if classically-secure one-way puzzles (OWPuzzs) exist. As far as we know, this is the first time that a complete cryptographic characterization of quantum advantage is obtained. IV-PoQ capture various types of quantum advantage previously studied, such as sampling-based quantum advantage and searching-based one. Previous work [Morimae and Yamakawa, Crypto 2024] showed that IV-PoQ can be constructed from OWFs, but a construction of IV-PoQ from weaker assumptions was left open. Our result solves the open problem. OWPuzzs are one of the most fundamental quantum cryptographic primitives implied by many quantum cryptographic primitives weaker than one-way functions (OWFs). The equivalence between IV-PoQ and classically-secure OWPuzzs therefore highlights that if there is no quantum advantage, then these fundamental primitives do not exist. The equivalence also means that quantum advantage is an example of the applications of OWPuzzs. Except for commitments, no application of OWPuzzs was known before. Our result shows that quantum advantage is another application of OWPuzzs, which solves the open question of [Chung, Goldin, and Gray, Crypto 2024]. Moreover, it is the first quantum-computation-classical-communication (QCCC) application of OWPuzzs.

==> Kolmogorov.tex <==
\section{Kolmogorov Complexity}
\label{sec:Kolmogorov} 
\takashi{I think at least the definitions and the statements of the lemmas should be given in the main body since they are not standard in cryptography (or quantum computing) and we use them in the main body in a crucial way. I think it's fine to move the proof of the lemmas to appendix.
}
\mor{In this Appendix, we... wo saisyoni kaku}
In this Appendix, we introduce the definition of time-bounded prefix Kolmogorov complexity and prove lemmas we have used in the proof of \Cref{lem:QAS_IVPoQ}.

A set $S\subseteq\bit^*$ of strings is called prefix-free, if any $x\in S$ is not a prefix of any other $y\in S$.
A function $t:\mathbb{N}\to\mathbb{N}$ is called time-constructible if $t(\secp)\ge\secp$ and there exists a Turing machine that takes $x\in\bit^\secp$ as input and outputs a binary representation of $t(|x|)$ in time $t(|x|)$.\mor{what is $x$?}

Time-bounded prefix Kolmogorov complexity is defined using a special type of Turing machines called \emph{self-delimiting machines}. 
For the purpose of this paper, we do not need to recall its definition in full detail (for which we refer to \cite[Chapter 3]{LV19}), and we only provide a brief explanation.   
Roughly, a self-delimiting machine is a Turing machine with a read-only \takashi{I added read-only} one-way input tape that initially contains only 0's and 1's with no blanks, a read-only two-way \takashi{I changed it to two-way. (This is not written in LV19 and I think either is fine, but two-way would be more natural.)} auxiliary tape, 
a two-way work tape, and a write-only one-way output tape.\footnote{\mor{Here, one-way means... two-way means...}
    Here, one-way means the tape head can only move in one direction, say from left to right, and two-way means the tape head can move in both directions.
} A self-delimiting machine $M$ takes as input a program $p$ in the input tape and an auxiliary input $y$ in the auxiliary tape. Its output is defined to be $x$ if, when $M$ halts, the output tape contains $x$ and the head of the input tape is on the rightmost bit of $p$ (which in particular means that $M$ never scans the next bit after $p$). We denote this by $M(p,y)=x$, and when $y$ is a null string, we simply write $M(p)=x$.   
%The only property of self-delimiting machines which we need is that if $M$ is a self-delimiting machine, then 
For a self-delimiting machine $M$ and an auxiliary input $y\in\bit^*$, we say that $p\in\bit^*$ is a valid program for $M$ with $y$ if there exists $x\in\bit^*$ such that $M(p,y)=x$.
For any self-delimiting machine $M$ and an auxiliary input $y$, the set of all valid programs $p\in\bit^*$ for $M$ with auxiliary input $y$
%  (i.e., $p$ such that $M(p,y)=x$ for some $x$) 
is prefix-free. 
\mor{i.e., ika ga valid no definition? Wakarinikuinode, waketekaku. Mazu valid no teigi wo suru. Tsugini valid natokiha prefix-free to iu.}
\takashi{I slightly modified the explanations. Please correct me if there's anything wrong.}
\begin{definition}[Time-Bounded Prefix Kolmogorov Complexity with respect to $M$ \cite{LV19}]
    Let $M$ be a self-delimiting machine.\mor{uedewa self-delimiting machine to nodeiru. touitsu suru}
    Let $t:\mathbb{N}\to\mathbb{N}$ be a time-constructible function and let $x,y\in\bit^*$.
    The $t$-time bounded prefix Kolmogorov complexity $K^t_M(x)$ with respect to $M$ is
    \begin{align}
        K^t_M(x) := \min \{ |p| : M(p)=x \text{~in at most $t(|x|)$ steps} \}.
    \end{align}
    Similarly, the $t$-time-bounded conditional prefix Kolmogorov complexity $K^t_M(x|y)$ with respect to $M$ is 
    \begin{align}
        K^t_M(x|y) := \min \{ |p| : M(p,y)=x \text{~in at most $t(|x|)$ steps} \}.
    \end{align} 
    \takashi{Meaning of $M(p,y)$ is unclear to me. Does this mean that $M$ takes a concatenation of $p$ and $y$, or it takes $y$ in an "auxiliary tape"? In the latter case, it is inconsistent to the definition of self-delimiting machine above.}
\end{definition}
\begin{remark}
There is another variant of time-bounded Kolmogorov complexity called time-bounded \emph{plain} Kolmogorov complexity where $M$ is a normal Turing machine rather than a self-delimiting one. Though the definition of the plain version is simpler than that of the above prefix version, we choose to use the prefix version since it is unclear if \Cref{lem:Kolm_prob} holds for the plain version (though we believe that we can prove a variant of \Cref{lem:Kolm_prob} for the plain version with some additional error terms, which would be also sufficient for the purpose of this paper). \takashi{I added this remark since this information will be very useful for non-experts in Kolmogorov complexity. Please correct me if there's anything wrong.}
\end{remark}

% \begin{lemma}[Efficient time-bounded invariance theorem (Example 7.1.1 of \cite{LV19})]\label{lem:Kolm_inv}
%     There is a universal self-delimiting machine $U$ that simulates all self-delimiting machines such that
%     for any self-delimiting machine $T$, there is a constant $c$ such that
%     \begin{align}
%         K^{ct\log t}_U(x|y) \le K^t_T(x|y) +c
%     \end{align}
%     holds for all $x,y\in\bit^*$.
% \end{lemma}

% This lemma implies the following corollary.
% \begin{corollary}\label{lem:conditional_Kolm}
%     Let $t$ be a time-constructible function.
%     For all $x,y\in\bit^*$ and any universal self-delimiting machine $U$ that satisfies the condition of \Cref{lem:Kolm_inv}, 
%     \takashi{Does this really work for "any" universal self-delimiting machine? Shouldn't that satisfy the condition of the above lemma?}\shira{fixed}
%     there exists a constant $c$ such that
%     \begin{align}
%         K^{ct\log t}_U (x|y) \le K^t_U(x) + c.
%     \end{align}
% \end{corollary}
% \begin{proof}[Proof of \cref{lem:conditional_Kolm}]
% Fix a universal self-delimiting machine $U$.
% Construct a self-delimiting machine $T$ that takes $(p,y)$ as input and runs $U(p)$.
% Then, for all $x,y\in\bit^*$, there is a constant $c'$ such that $K^t_T(x|y)\le K^t_U(x)+c'$.
% By \Cref{lem:Kolm_inv}, we obtain $K^{ct\log t}_U(x|y)\le K^t_T(x|y)+c\le K^t_U(x)+c+c'$.
% \end{proof}

\begin{definition}[\cite{LV19}]
    Let $P:\bit^*\to[0,1]$ be a function.
    If there exists a Turing machine that on input $x$ and a positive integer $k$ computes a rational number $y$ in at most $t(n+k)$ steps,
    where $n=|x|$, such that $|P(x)-y|\le\frac{1}{2^k}$ for any $x$ and $k$, then we say that
    $P$ is computable in time $t(n)$.
    \mor{what is $n$? It is defined later, but it is not clear at this stage. This must be clear at this stage.} 
    \mor{for any $x$ and $k$?}
\end{definition}

\shira{I added the following.}
Universal self-delimiting machines are self-delimiting machines that can simulate any other self-delimiting machines.
We can construct a universal self-delimiting machine $U$ as follows:
$U$ has a one-way read-only input tape whose prefix is $1^n\|0\|p$, an auxiliary tape with $y$, work tapes, and an output tape.
\mor{A and B and C and... wa bunpoutekini okashiinodewa?}
$U$ runs $M_n(p,y)$, where $M_1,M_2,...$ is an enumeration of all self-delimiting machines.

There are several ways to construct universal self-delimiting machines, but in this paper, we focus on the above one and we call $U$ the universal self-delimiting machine.

% \begin{lemma}[Claim 7.6.1 of \cite{LV19}]
% Let $U$ be a universal self-delimiting machine.
%     Let $\{p_y\}_{y\in\bit^n}$ be a distribution and let $p^*_y := \sum_{x\le y} p_x$, where $x\le y$ means $x$ is lexicographically smaller than $y$. \takashi{What order do you consider for bit strings?}\shira{fixed}
%     If $p^*_y$ is computable in time $t'(n)$ for all $y\in\bit^n$, then there are a function
%     $t$ such that
%     $t(n)=O(nt'(n)\log(nt'(n)))$
%     and a constant $c$ such that for all $y\in\bit^n$,
%     \begin{align}
%         K^{t}_U(y) \le \log \frac{1}{p_y} + c,
%     \end{align}
% \end{lemma}

\begin{lemma}\label{lem:Kolm_bound}
    Let $U$ be the universal self-delimiting \mor{Turing ga tuitari tukanakattari. Touitsusuru} machine. 
    Let $\{p_x\}_{x\in\bit^n}$ be a distribution and let $p^*_x := \sum_{z\le x} p_z$, where $z\le x$ means $z$ is lexicographically smaller than $x$. 
    If $p^*_x$ is computable in time $t'(n)$ for all $x\in\bit^n$, then there exist a function $t$ such that $t(n)=O(nt'(n)\log^2(nt'(n)))$ and a constant $c>0$ \mor{$c>0$?} such that for all $x\in\bit^n$ and all $y\in\bit^*$,
    \begin{align}
        K^{t}_U(x|y) \le \log \frac{1}{p_x} + c.
   \end{align}
\end{lemma}
\begin{proof}[Proof of \Cref{lem:Kolm_bound}]
By Example 7.1.1 of \cite{LV19}\footnote{
    In \cite{LV19}, only the case of unconditional prefix Kolmogorov complexity is mentioned, but it can be generalized to the conditional case.
}, $U$ satisfies the following:
For any self-delimiting machine $M$, there exists a constant $c_1$ such that for all $x,y\in\bit^*$ and for any time-constructible function $t$,
\begin{align}\label{eq:optimal}
    K^{c_1t\log t}_U(x|y) \le K^t_M(x|y)+c_1.
\end{align}
Consider the self-delimiting Turing machine $M^*$ that on input $(p,y)$, ignores $y$ and runs $U(p)$.
Then, $K^t_{M^*}(x|y)=K^t_U(x)$ holds for all $x,y\in\bit^*$ and any time-constructible function $t$.
\Cref{eq:optimal} holds for $M^*$ and therefore, there exists a constant $c_2$ such that for all $x,y\in\bit^*$ and for any time-constructible function $t$,
\begin{align}\label{eq:conditional}
    K^{c_2t\log t}_U(x|y) \le K^t_U(x) + c_2.
\end{align}
Let $p^*_x$ be computable in time $t'(n)$ for all $x\in\bit^n$.
By Claim 7.6.1 of \cite{LV19}, there exist a function $t$ such that $t(n)=O(nt'(n)\log(nt'(n)))$ and a constant $c_3$ such that for all $x\in\bit^n$,
\begin{align}\label{eq:coding}
    K^t_U(x) \le \log\frac{1}{p_x} +c_3.
\end{align}
By combining \Cref{eq:conditional,eq:coding}, there exist a function $t$ such that $t(n)=O(nt'(n)\log(nt'(n)))$ and constants $c_2$ and $c_3$ such that for all $x\in\bit^n$ and for all $y\in\bit^*$, 
\begin{align}
    K^{c_2t\log t}_U(x|y) \le \frac{1}{p_x} + c_2+c_3.
\end{align}
Then, $c_2t(n)\log t(n)=O(t(n)\log t(n))=O(nt'(n)\log^2(nt'(n)))$ and therefore we complete the proof.

\end{proof}

\begin{lemma}\label{lem:Kolm_prob}
Let $U$ be the universal self-delimiting machine.
    Let $\cD=\{p_x\}_{x\in\bit^*}$ be any distribution. For any $k>0$,
    \begin{align}
        \Pr_{x\gets\cD} \left[K^t_U(x)\ge \log\frac{1}{p_x}-k\right] \ge 1-\frac{1}{2^k}.
    \end{align}
    Moreover, for any $y\in\bit^*$ and for any $k>0$,
    \begin{align}
        \Pr_{x\gets\cD} \left[ K^t_U(x|y) \ge \log\frac{1}{p_x}-k \right] \ge 1-\frac{1}{2^k}.
    \end{align}
\end{lemma}
\begin{proof}[Proof of \cref{lem:Kolm_prob}]
For any $x\in\bit^*$, let $P_x$ be a program such that $U(P_x)$ outputs $x$ in at most $t(|x|)$ steps and $|P_x|=K^t_U(x)$.  
Then, the set $\{P_x\}_{x\in\bit^*}$ is prefix-free since $U$ is a self-delimiting machine. 
It is known that 
    $\sum_{x\in\bit^*} 2^{-|P_x|} \le 1$
holds for prefix-free $\{P_x\}_{x\in\bit^*}$. (It is called Kraft's inequality~\cite{LV19}.)
By Markov's inequality,
\begin{align}
    \Pr_{x\gets\cD} \left[ \frac{2^{-K^t_U(x)}}{p_x} \ge 2^k \right]
    \le \frac{1}{2^k} \sum_x p_x \frac{2^{-K^t_U(x)}}{p_x} 
    = \frac{1}{2^k} \sum_x 2^{-K^t_U(x)} 
    = \frac{1}{2^k} \sum_x 2^{-|P_x|}
    \le \frac{1}{2^k}.
\end{align}
Therefore, we obtain
\begin{align}
    \Pr_{x\gets\cD} \left[K^t_U(x)\ge \log\frac{1}{p_x}-k\right] \ge 1-\frac{1}{2^k}.
\end{align}
The same proof holds for the case of $K^t_U(x|y)$ because the set $\{P'_x\}_{x\in\bit^*}$ such that $U(P'_x,y)$ outputs $x$ in at most $t(|x|)$ steps and $|P'_x|=K^t_U(x|y)$ is also prefix-free.

\end{proof}
